Large Language Models Fall Short: Understanding Complex Relationships in Detective Narratives

Existing datasets for narrative understanding often fail to represent the complexity and uncertainty of relationships in real-life social scenarios. To address this gap, we introduce a new benchmark, Conan, designed for extracting and analysing intricate character relation graphs from detective narratives. Specifically, we designed hierarchical relationship categories and manually extracted and annotated role-oriented relationships from the perspectives of various characters, incorporating both public relationships known to most characters and secret ones known to only a few. Our experiments with advanced Large Language Models (LLMs) like GPT-3.5, GPT-4, and Llama2 reveal their limitations in inferencing complex relationships and handling longer narratives. The combination of the Conan dataset and our pipeline strategy is geared towards understanding the ability of LLMs to comprehend nuanced relational dynamics in narrative contexts.

==> Sections/v2_introduction.tex <==
\section{Introduction}\label{sec:intro}


Recently, many studies have been conducted to evaluate the cognitive abilities of LLMs. Some claim that LLMs perform better than the average human being \citep{bubeck2023gpt4AGI}, while others argue that LLMs are merely reproducing what they have previously encountered and are not truly capable of understanding the content \citep{qin2023llm-problemsolver, West2023AIparadox}. Boosted by the impressive capabilities of LLMs, tasks like multi-agent interaction \citep{generative-agent2023, werewolf2023, avalon2023} and narrative understanding \citep{Zhu2023AreNM} have recently gained significant attention. These tasks require a deeper understanding of complex, potentially evolving relationships between multiple entities \citep{worth2004narrative}. 
% 错误的关系认知会怎样影响用户体验？？related works
Detective stories, with characters often possessing multiple identities or aliases revealed at various points, align perfectly with these requirements.

\begin{figure*}[th!]
    \centering
    \includegraphics[width=\linewidth]{setting.pdf}
    \caption{}
    \label{fig:examples}
\end{figure*}


Previous research exploring the narrative comprehension and inferential abilities of LLMs have typically based on question answering \cite{yang2019friendsQA, xu-etal-2022-fantastic, gandhi2023bigtom}, which may include questions about relations but do not cover all character relationships. 
Research has been conducted on extracting relationships directly from sentences \cite{you2020relation-trajectories, mallace2020relation-clustering}, , typically focusing on verbs, such as \emph{say}, \emph{smile}, \emph{look}. However, these are not the types of relationships we are interested in; we aim to understand higher-level relationships, such as familial ties, friendships, etc. Recent work \citep{chen2023harrypotter} has annotated relationships among Harry Potter characters. However, like earlier datasets, their corpus tends to be straightforward, with few examples of false identities, ambiguous identity references \citep{narrativeplay2023}, such as just an appearance description from the other character's perspective: \emph{``A middle-aged man quickly walked out of the main gate, with grey and white hair, and a slender build. ''}, or conflicting understandings of the same relationship from different perspectives.
%or relies on corpora whose complexity or quality \citep{le2019revisiting} no longer meet the current needs for evaluation or training. 
%Existing works to investigate the cognitive and inferential abilities on LLMs are either not focusing on entity relationships, or the corpus being artificially made and does not fit for what is needed today.
%At the same time, as a highly challenging task, it has also become a suitable 

Therefore, we construct FatalWeb, a dataset designed for extracting role-oriented relation graphs from detective narratives. This dataset can act as a benchmark to test the cognitive and inferential abilities of LLMs. Additionally, it holds the potential to improve LLM capabilities in areas such as narrative comprehension \citep{narrativeplay2023}, simulation agents \citep{generative-agent2023}, and game agents \citep{werewolf2023, avalon2023}.

%Limitations:
LLMs are found being capable of generating the relationships stated in narrative but not able to understand the relationships. As we shown in Figure~\ref{fig:examples}, it is struggle to understand the complex role relation in narrative: 
%We found that LLMs are capable of generating the relationships stated in narrative but not able to understand the relationships. As we shown in Figure~\ref{fig:examples}, it somethings missing the obvious relationship due to the reversal curse \citep{}.
For quantitative results, we conducted tests using our benchmark on three cutting-edge Large Language Models (GPT-3.5, GPT-4, and Llama2-chat), and our findings reveal that these models face difficulties in managing character relationships within detective narratives.


In response to the identified challenges, we propose a pipeline framework aimed at constructing a relation graph for each character's perspective. This framework is designed to minimise the impact of long input \citep{liu2023lost-in-the-middle} and enhance the accuracy of their responses. We first determine if a relationship contains contradictions, which allows for the straightforward merging of entities and relations without conflicts. Subsequently, we employ RAG\footnote{\url{https://github.com/weaviate/Verba}} to retrieve evidence, in order to enhance attention to key information, thereby refining the model's comprehension of contradictory information from diverse perspectives and improving the consistency of its outputs. Finally, we classify the conflict scenarios and record the classification result as the refined relationship.



%Finally, we propose a pipeline framework for the challenge, that build-up the relation graph for each perspective. In order to reduce the model's hallucinations and ensure the accuracy of its answers, we first identify whether the relationship contains a contradiction. Therefore, we can easily merge the entities and relations that do not have conflicts. Then, we retrieve evidence based on RAG\footnote{\url{https://github.com/weaviate/Verba}} to enhance attention to key information to improve the model's understanding of contradictory information from different perspectives and the consistency of its outputs. Then, we classify on the conflict options and save the classification result as the refined relation. %We then get the relationship graphs which can be used to verify and store relationships between people, % and factual knowledge, 


%As studied by \citet{}, LLMs are easily lost in the middle, therefore, when 
%theory of mind - ToMi is 

In summary, we have made the following contributions:
\begin{itemize}[noitemsep,nolistsep]
    \item We present the FatalWeb dataset, created to evaluate and enhance the capacity of LLMs to comprehend intricate relationships in detective narratives. 

    \item We conducted tests using our benchmark on three cutting-edge Large Language Models (GPT-3.5, GPT-4, and Llama2), and our findings reveal that these models face difficulties in managing character relationships within detective narratives.
    
    \item We proposed a pipeline framework that utilises RAG to enhance the inferential capabilities of LLMs, particularly in identifying and addressing contradictions within character relationships. 
\end{itemize}

